Electric Field Gradient Calculations for Ice VIII and IX using Polarizable Embedding: A Comparative Study on Classical Computers and Quantum Simulators

We test the performance of the Polarizable Embedding Variational Quantum Eigensolver Self-Consistent-Field (PE-VQE-SCF) model for computing electric field gradients with comparisons to conventional complete active space self-consistent-field (CASSCF) calculations and experimental results. We compute quadrupole coupling constants for ice VIII and ice IX. We find that the inclusion of the environment is crucial for obtaining results that match the experimental data. The calculations for ice VIII are within the experimental uncertainty for both CASSCF and VQE-SCF for oxygen and lie close to the experimental value for ice IX as well. With the VQE-SCF, which is based on an Adaptive Derivative-Assembled Problem-Tailored (ADAPT) ansatz, we find that the inclusion of the environment and the size of the different basis sets do not directly affect the gate counts. However, by including an explicit environment, the wavefunction and, therefore, the optimization problem becomes more complicated, which usually results in the need to include more operators from the operator pool, thereby increasing the depth of the circuit.

==> tables/ice8_itervscnot.tex <==
\begin{table}[h!]
\centering 
\caption{Ice VIII. CNOT counts and the number of iterations until convergence, averaged over the calculations for the different water molecules in the unit cell.}
\label{tab:ice8_itervscnot}
\small
\begin{tabular}{lcccc} \toprule 
& Vacuum & Vacuum & Embedded & Embedded\\
Basis & Iterations & CNOT & Iterations & CNOT\\[1.0ex]


\hline6-311++G & 42 & 4260 & 46 & 4863 \\ [1.0ex]
6-311++G** & 50 & 5184 & 51 & 5186 \\ [1.0ex]
cc-pCVDZ & 41 & 4464 & 69 & 7470 \\ [1.0ex]
cc-pCVTZ & 72 & 7875 & 84 & 8718 \\ [1.0ex]
aug-cc-pCVDZ & 27 & 2223 & 31 & 2949 \\ [1.0ex]
aug-cc-pCVTZ & 46 & 4484 & 44 & 4470 \\ [1.0ex]


\bottomrule \end{tabular}\end{table} \normalsize

==> tables/ice8energydev.tex <==

\begin{table}[ht!]
\centering 
\caption{Ice VIII. Deviations of the PE-VQE-SCF energies from the CASSCF results in mEh.}
\label{tab:ice8energydev}
\small
\begin{tabular}{rccccc} \toprule 
Basis & Mean dev & Abs. dev & Standard dev & Max dev & Min dev\\[1.0ex]


\hline6-311++G & 0.957 & 0.957 & 0.077 & 1.114 & - \\ [1.0ex]
6-311++G** & 1.245 & 1.245 & 0.231 & 1.413 & - \\ [1.0ex]
cc-pCVDZ & $-7.71$ & 7.71 & 12.863 & - & $-29.146$ \\ [1.0ex]
cc-pCVTZ & $-7.201$ & 8.101 & 14.447 & 0.989 & $-30.612$ \\ [1.0ex]
aug-cc-pCVDZ & $-2.308$ & 2.308 & 0.122 & - & $-2.429$ \\ [1.0ex]
aug-cc-pCVTZ & $-1.053$ & $-1.139$ & $-1.303$ & $-1.341$ & $-1.389$ \\ [1.0ex]







\bottomrule \end{tabular}\end{table} \normalsize

==> tables/ice9_itervscnot.tex <==
\begin{table}[h!]
\centering 
\caption{Ice IX. CNOT counts and the number of iterations until convergence, averaged over the calculations for the different water molecules in the unit cell.}
\label{tab:ice9_itervscnot}
\small
\begin{tabular}{lcccc} \toprule 
& Vacuum & Vacuum & Embedded & Embedded\\
Basis & Iterations & CNOT & Iterations & CNOT\\[1.0ex]


\hline6-311++G & 37 & 3863 & 55 & 6345 \\ [1.0ex]
6-311++G** & 46 & 4940 & 67 & 7028 \\ [1.0ex]
cc-pCVDZ & 44 & 4861 & 84 & 8894 \\ [1.0ex]
cc-pCVTZ & 66 & 7211 & 84 & 8288 \\ [1.0ex]
aug-cc-pCVDZ & 28 & 2650 & 45 & 4868 \\ [1.0ex]
aug-cc-pCVTZ & 47 & 4735 & 51 & 5340 \\ [1.0ex]






\bottomrule \end{tabular}\end{table} \normalsize

==> tables/ice9energydev.tex <==

\begin{table}[ht!]
\centering 
\caption{Ice IX. Deviations of the PE-VQE-SCF energies from the CASSCF results in mEh.}
\label{tab:ice9energydev}
\small
\begin{tabular}{rccccc} \toprule 
Basis & Mean dev & Abs. dev & Standard dev & Max dev & Min dev\\[1.0ex]


\hline6-311++G & 2.318 & 2.318 & 0.159 & 2.737 & - \\ [1.0ex]
6-311++G** & -0.435 & 1.212 & 2.923 & 0.926 & -9.667 \\ [1.0ex]
cc-pCVDZ & -0.686 & 1.047 & 2.717 & 0.618 & -9.246 \\ [1.0ex]
cc-pCVTZ & 2.515 & 2.515 & 1.817 & 4.61 & - \\ [1.0ex]
aug-cc-pCVDZ & -0.702 & 1.404 & 2.925 & 0.926 & -9.667 \\ [1.0ex]
aug-cc-pCVTZ & 20.907 & 20.907 & 12.286 & 29.028 & - \\ [1.0ex]





\bottomrule \end{tabular}\end{table} \normalsize
